Unsupervised Video Interpolation by Learning Multilayered 2.5D Motion Fields

The problem of video frame interpolation is to increase the temporal resolution of a low frame-rate video, by interpolating novel frames between existing temporally sparse frames. This paper presents a self-supervised approach to video frame interpolation that requires only a single video. We pose the video as a set of layers. Each layer is parameterized by two implicit neural networks -- one for learning a static frame and the other for a time-varying motion field corresponding to video dynamics. Together they represent an occlusion-free subset of the scene with a pseudo-depth channel. To model inter-layer occlusions, all layers are lifted to the 2.5D space so that the frontal layer occludes distant layers. This is done by assigning each layer a depth channel, which we call `pseudo-depth', whose partial order defines the occlusion between layers. The pseudo-depths are converted to visibility values through a fully differentiable SoftMin function so that closer layers are more visible than layers in a distance. On the other hand, we parameterize the video motions by solving an ordinary differentiable equation (ODE) defined on a time-varying neural velocity field that guarantees valid motions. This implicit neural representation learns the video as a space-time continuum, allowing frame interpolation at any temporal resolution. We demonstrate the effectiveness of our method on real-world datasets, where our method achieves comparable performance to state-of-the-arts that require ground truth labels for training.

==> Comparisons/fig_comparison.tex <==
\captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}[b]{0.135\textwidth}
% \captionsetup[subfigure]{labelformat=empty}
%     %\vspace*{0.8ex}
%     \includegraphics[width=\textwidth]{Comparisons/DogDance1.png}
    
%     \vspace{0.81ex}
%      \includegraphics[width=\textwidth]{Comparisons/DogDance2.png}
% \caption{Inputs}
% \end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_dain.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{DAIN\cite{bao2019depth}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_toflow.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{TOFlow\cite{xue2019video}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_abme.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{ABME\cite{park2021asymmetric}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_rife.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{RIFE\cite{huang2020rife}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_rife.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{CC\cite{reda2019unsupervised}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_ours.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_gt.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{G.T.}
\end{subfigure}



==> Comparisons/fig_comparison_2.tex <==
\captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}[b]{0.135\textwidth}
% \captionsetup[subfigure]{labelformat=empty}
%     %\vspace*{0.8ex}
%     \includegraphics[width=\textwidth]{Comparisons/Venus1.png}
    
%     \vspace{0.81ex}
%      \includegraphics[width=\textwidth]{Comparisons/Venus2.png}


% \caption{Inputs}
% \end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]  
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_dain.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{DAIN\cite{bao2019depth}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_toflow.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{TOFlow\cite{xue2019video}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_abme.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{ABME\cite{park2021asymmetric}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_rife.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{RIFE\cite{huang2020rife}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_rife.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{CC\cite{reda2019unsupervised}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_ours.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_gt.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{G.T.}
\end{subfigure}
\captionsetup[subfigure]{labelformat=simple}

==> VFI ECCV/Comparisons/fig_comparison.tex <==
\captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}[b]{0.135\textwidth}
% \captionsetup[subfigure]{labelformat=empty}
%     %\vspace*{0.8ex}
%     \includegraphics[width=\textwidth]{Comparisons/DogDance1.png}
    
%     \vspace{0.81ex}
%      \includegraphics[width=\textwidth]{Comparisons/DogDance2.png}
% \caption{Inputs}
% \end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_dain.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{DAIN\cite{bao2019depth}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_toflow.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{TOFlow\cite{xue2019video}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_abme.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{ABME\cite{park2021asymmetric}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_rife.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{RIFE\cite{huang2020rife}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_rife.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{CC\cite{reda2019unsupervised}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_ours.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=2, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/DogDance_gt.png} };
    \zoombox[magnification=4,color code=green]{0.6,0.13}
    \zoombox[magnification=1.5]{0.75,0.4}
\end{tikzpicture}
\vspace{-2.5em}
\caption{G.T.}
\end{subfigure}



==> VFI ECCV/Comparisons/fig_comparison_2.tex <==
\captionsetup[subfigure]{labelformat=empty}
% \begin{subfigure}[b]{0.135\textwidth}
% \captionsetup[subfigure]{labelformat=empty}
%     %\vspace*{0.8ex}
%     \includegraphics[width=\textwidth]{Comparisons/Venus1.png}
    
%     \vspace{0.81ex}
%      \includegraphics[width=\textwidth]{Comparisons/Venus2.png}


% \caption{Inputs}
% \end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]  
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_dain.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{DAIN\cite{bao2019depth}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_toflow.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{TOFlow\cite{xue2019video}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_abme.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{ABME\cite{park2021asymmetric}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_rife.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{RIFE\cite{huang2020rife}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_rife.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{CC\cite{reda2019unsupervised}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_ours.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=1]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Venus_gt.png} };
    \zoombox[magnification=7,color code=green]{0.81,0.37}
\end{tikzpicture}
\vspace{-2.5em}
\caption{G.T.}
\end{subfigure}
\captionsetup[subfigure]{labelformat=simple}

==> VFI ECCV/Comparisons/fig_comparison_combined.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{DAIN\cite{bao2019depth}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{TOFlow\cite{xue2019video}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\vspace{-0em}
\caption{ABME\cite{park2021asymmetric}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{RIFE\cite{huang2020rife}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{CC\cite{reda2019unsupervised}}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\vspace{-0em}
\caption{G.T.}
\end{subfigure}



==> VFI ECCV/Comparisons/flounder.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{minipage}{0.45\textwidth}
\begin{subfigure}{\textwidth}
\raisebox{-\height}{\includegraphics[width=0.49\textwidth]{Comparisons/0085_0.png}}
\raisebox{-\height}{\includegraphics[width=0.49\textwidth]{Comparisons/0085_1.png}}

\vspace*{0.05ex}
\raisebox{-\height}{\includegraphics[width=0.49\textwidth]{Comparisons/0085_2.png}}
\raisebox{-\height}{\includegraphics[width=0.49\textwidth]{Comparisons/0085_3.png}}
\vspace*{-0.25ex}
\caption{per-layer frames}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\begin{subfigure}[b]{\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\includegraphics[width=\textwidth]{Comparisons/0085.png}
\caption{blended frame}
\end{subfigure}
\end{minipage}




==> VFI ECCV/Comparisons/grove.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_8.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{8 frames}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_6.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{6 frames}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_4.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{4 frames}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_2.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{2 frames}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_2_ref.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{2 frames{\tiny (reg.$\uparrow$)}}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\begin{tikzpicture}[zoomboxarray, zoomboxes below, zoomboxarray columns=1, zoomboxarray rows=2]
    \tiny
    \node [image node] { \includegraphics[width=\textwidth]{Comparisons/Grove2_gt.png} };
    \zoombox[magnification=2.5,color code=green]{0.4,0.72}
\end{tikzpicture}
\vspace*{-1.9cm}
\caption{G.T.}
\end{subfigure}



==> VFI ECCV/Comparisons/rubberwhale.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}[b]{0.23\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\includegraphics[width=\textwidth]{Comparisons/layer1.png}
\caption{1-layer model}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\includegraphics[width=\textwidth]{Comparisons/layer2.png}
\caption{2-layer model}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\includegraphics[width=\textwidth]{Comparisons/layer3.png}
\caption{3-layer model}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\captionsetup[subfigure]{labelformat=empty}
\includegraphics[width=\textwidth]{Comparisons/layer4.png}
\caption{4-layer model}
\end{subfigure}




==> VFI ECCV/Networks/FNet.tex <==
\begin{tikzpicture}[
squarednode/.style={rectangle, rounded corners=3, draw=black, very thick, minimum height=1cm, align=center},
delta_t_wrap/.style={rectangle, rounded corners=3, draw=black, thick, align=center, dotted},
dashedsquarednode/.style={rectangle, dashed, rounded corners=6, draw=black, thick, minimum size=5mm},
arrow_text/.style={thick, font=\small},
text_box/.style={rectangle, font=\small},
background_box/.style={rounded corners=6, dashed, thick, color=green(pigment)},
]

%background
\fill[fill=red!5, rounded corners=12](-3.25,-2.75) rectangle (0.5, 3);
\fill[fill=red!5](0,-2.75) rectangle (0.5, 3);
\fill[fill=blue!5](0.5, 3) rectangle (1, -2.75);
\fill[fill=blue!5, rounded corners=12](0.5, 3) rectangle (3.85, -2.75);
%nodes
\node[dashedsquarednode,minimum height=4mm] (input) at (-4,0) {$u_F,v_F$};
\node[squarednode, minimum width=1.1cm, minimum height=3cm] (pos_enc)     at(-2.5, 0)   {\\\\\\\\ Pos. \\ Enc.};

\draw[very thick](-2.5,0.6) circle (0.4);
\draw[blue, very thick] (-2.85, 0.6) sin (-2.675,0.8) cos (-2.5,0.6) sin (-2.325,0.4) cos (-2.15,0.6);

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer1)     at(-1.25, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}Sinusoidal};

%\draw[thick, ->] (2.05,2) arc (-55:240:0.8);
%\node[rectangle] at(1.6, 2.7) {$t=1..T$};

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer2)     at(-0.25, 0)   {(...)};

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer3)     at(1.25, 0)   {(...)};

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer4)     at(2.25, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}Sinusoidal};

\node[squarednode, minimum width=3.5cm, minimum height=0.7cm, rotate=90] (fc_layer5)     at(3.25, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}Sigmoid};


\node[dashedsquarednode,minimum height=4mm] (output) at (5,0) {$R,G,B,D$};
% text box

\node[rectangle] at(-1.25, 2) {$256$};
\node[rectangle] at(-0.25, 2) {$256$};
\node[rectangle] at(1.25, 2) {$256$};
\node[rectangle] at(2.25, 2) {$256$};
\node[rectangle] at(3.25, 1.5) {$4$};


%arrows
\draw[->, arrow_text, very thick] (input.east) -- (pos_enc.west);
\draw[->, arrow_text, very thick] (pos_enc.east) -- (fc_layer1.north);
\draw[->, arrow_text, very thick] (fc_layer1.south) -- (fc_layer2.north);
\draw[->, arrow_text, very thick] (fc_layer2.south) -- (fc_layer3.north);
\draw[->, arrow_text, very thick] (fc_layer3.south) -- (fc_layer4.north);
\draw[->, arrow_text, very thick] (fc_layer4.south) -- (fc_layer5.north);
\draw[->, arrow_text, very thick] (fc_layer5.south) -- (output.west);
% curly brace
\draw[decoration={brace,raise=5pt},decorate, thick] (-1.5,2.2) -- node[above=6pt] {$4$ layers} (0,2.2);
\draw[decoration={brace,raise=5pt},decorate, thick] (1,2.2) -- node[above=6pt] {$4$ layers} (2.5,2.2);
\end{tikzpicture}

==> VFI ECCV/Networks/MNet.tex <==
\begin{tikzpicture}[
squarednode/.style={rectangle, rounded corners=3, draw=black, very thick, minimum height=1cm, align=center},
delta_t_wrap/.style={rectangle, rounded corners=3, draw=black, thick, align=center, dotted},
dashedsquarednode/.style={rectangle, dashed, rounded corners=6, draw=black, thick, minimum size=5mm},
arrow_text/.style={thick, font=\small},
text_box/.style={rectangle, font=\small},
background_box/.style={rounded corners=6, dashed, thick, color=green(pigment)},
]

%background
\fill[fill=blue!5, rounded corners=12](-3.25,-2.75) rectangle (4, 3);

%nodes
\node[dashedsquarednode, minimum height=0.45cm] (input)     at(-4, 0.25)   {$u_i,v_i$};
\node[dashedsquarednode, minimum height=0.45cm] (t_input)     at(-3.5, -0.25)   {$t_i$};

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer1)     at(-2, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}L.ReLU};

\node[squarednode, minimum width=4.5cm, minimum height=0.7cm, rotate=90] (fc_layer2)     at(-1, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}L.ReLU};


\node[squarednode, minimum width=3cm, minimum height=0.7cm, rotate=90] (fc_layer3)     at(0, 0)   {FC\hspace{0.3cm}+\hspace{0.3cm}tanh};

\node[rectangle, font=\huge, inner sep=0pt] (concat_syl) at(1.45, 0) {$\oplus$};

\node[dashedsquarednode, minimum height=0.45cm] (output)     at(3, 0)   {$u_{i+1},v_{i+1}$};
% text box
\node[rectangle] at(-2, 2) {$256$};
\node[rectangle] at(-1, 2) {$256$};
\node[rectangle] at(0, 1.25) {$2$};


%arrows
\draw[->, arrow_text,very thick] (t_input.east) -- ($(fc_layer1.north)+(0,-0.25)$);
\draw[->, arrow_text,very thick] ($(input.east)+(-0.1,0)$) -- ($(fc_layer1.north)+(0,0.25)$);
\draw[->, arrow_text,very thick] (fc_layer1.south) -- (fc_layer2.north);
\draw[->, arrow_text,very thick] (fc_layer2.south) -- (fc_layer3.north);
\draw[->, arrow_text,very thick] (fc_layer3.south) -- ($(concat_syl.west)+(0.05,0)$);
\path[arrow_text] (fc_layer3.south) -- ($(concat_syl.west)+(0.05,0)$) node[midway,above] {$\times\Delta t$};

\draw[->, arrow_text,very thick] ($(concat_syl.east)+(-0.07,0)$) -- (output.west);
%\path[arrow_text] ($(concat_syl.east)+(-0.07,0)$) -- (2.25,0) node[midway,above] {$X_{i+1}$};

\draw[->, arrow_text,very thick] (input.south) to ($(input)+(0,-2.75)$) to ($(concat_syl)+(0,-2.5)$) to ($(concat_syl.south) + (0, 0.02)$);

\draw[->, arrow_text, color=blue,very thick] (output.north) to ($(output)+(0,2.5)$) to ($(input)+(0,2.25)$) to (input.north);
\path[arrow_text] (5.3, 2.35) -- ($(input)+(0,2.35)$) node[midway,above] {$t_{i+1}=t_i+\Delta t,\ i=i+1$};




\end{tikzpicture}

==> VFI ECCV/math_commands.tex <==


%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Added minimize
\DeclareMathOperator*{\minimize}{minimize}
% Add given
\newcommand\given[1][]{\:#1\vert\:}

% Inline row / column vector
\newcommand{\icol}[1]{% inline column vector
  \left(\begin{smallmatrix}#1\end{smallmatrix}\right)%
}

\newcommand{\irow}[1]{% inline row vector
  \begin{smallmatrix}(#1)\end{smallmatrix}%
}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\bepsilon{{\mathbf{\epsilon}}}
\def\btheta{{\mathbf{\theta}}}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\be{{\mathbf{e}}}
\def\bf{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bu{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\calA{{\mathcal{A}}}
\def\calB{{\mathcal{B}}}
\def\calC{{\mathcal{C}}}
\def\calD{{\mathcal{D}}}
\def\calE{{\mathcal{E}}}
\def\calF{{\mathcal{F}}}
\def\calG{{\mathcal{G}}}
\def\calH{{\mathcal{H}}}
\def\calI{{\mathcal{I}}}
\def\calJ{{\mathcal{J}}}
\def\calK{{\mathcal{K}}}
\def\calL{{\mathcal{L}}}
\def\calM{{\mathcal{M}}}
\def\calN{{\mathcal{N}}}
\def\calO{{\mathcal{O}}}
\def\calP{{\mathcal{P}}}
\def\calQ{{\mathcal{Q}}}
\def\calR{{\mathcal{R}}}
\def\calS{{\mathcal{S}}}
\def\calT{{\mathcal{T}}}
\def\calU{{\mathcal{U}}}
\def\calV{{\mathcal{V}}}
\def\calW{{\mathcal{W}}}
\def\calX{{\mathcal{X}}}
\def\calY{{\mathcal{Y}}}
\def\calZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Theorem environments
% Theorems, definitions, etc
%\def\thmcolon{\hspace{-.85em} {\bf :}}
\def\thmcolon{\relax}

% \newtheorem{THEOREM}{Theorem}
%\newtheorem{THEOREM}{Theorem}[section]
% \newtheorem{LEMMA}[THEOREM]{Lemma}
% \newtheorem{PROPOSITION}[THEOREM]{Proposition}
% \newtheorem{COROLLARY}[THEOREM]{Corollary}
% \newtheorem{DEFINITION}[THEOREM]{Definition}
% \newtheorem{OBSERVATION}[THEOREM]{Observation}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}

% Easiest way to remove the full stop and add a colon
% \usepackage{xpatch}
% \makeatletter
% \AtBeginDocument{\xpatchcmd{\@thm}{\thm@headpunct{.}}{\thm@headpunct{:}}{}{}}
% \makeatother

% \newenvironment{theorem}{\begin{THEOREM} \thmcolon \rm}{\end{THEOREM}}
% \newenvironment{lemma}{\begin{LEMMA} \thmcolon \rm}{\end{LEMMA}}
% \newenvironment{proposition}{\begin{PROPOSITION} \thmcolon \rm}{\end{PROPOSITION}}
% \newenvironment{corollary}{\begin{COROLLARY} \thmcolon \rm}{\end{COROLLARY}}
% \newenvironment{definition}{\begin{DEFINITION} \thmcolon \rm}{\end{DEFINITION}}
% \newenvironment{observation}{\begin{OBSERVATION} \thmcolon \rm}{\end{OBSERVATION}}


%%%%% ABBREVIATIONS %%%%%
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

==> VFI ECCV/zoombox.tex <==
\newif\ifblackandwhitecycle
\gdef\patternnumber{0}

\pgfkeys{/tikz/.cd,
    zoombox paths/.style={
        draw=orange,
        very thick
    },
    black and white/.is choice,
    black and white/.default=static,
    black and white/static/.style={ 
        draw=white,   
        zoombox paths/.append style={
            draw=white,
            postaction={
                draw=black,
                loosely dashed
            }
        }
    },
    black and white/static/.code={
        \gdef\patternnumber{1}
    },
    black and white/cycle/.code={
        \blackandwhitecycletrue
        \gdef\patternnumber{1}
    },
    black and white pattern/.is choice,
    black and white pattern/0/.style={},
    black and white pattern/1/.style={    
            draw=white,
            postaction={
                draw=black,
                dash pattern=on 2pt off 2pt
            }
    },
    black and white pattern/2/.style={    
            draw=white,
            postaction={
                draw=black,
                dash pattern=on 4pt off 4pt
            }
    },
    black and white pattern/3/.style={    
            draw=white,
            postaction={
                draw=black,
                dash pattern=on 4pt off 4pt on 1pt off 4pt
            }
    },
    black and white pattern/4/.style={    
            draw=white,
            postaction={
                draw=black,
                dash pattern=on 4pt off 2pt on 2 pt off 2pt on 2 pt off 2pt
            }
    },
    zoomboxarray inner gap/.initial=5pt,
    zoomboxarray columns/.initial=2,
    zoomboxarray rows/.initial=2,
    subfigurename/.initial={},
    figurename/.initial={zoombox},
    zoomboxarray/.style={
        execute at begin picture={
            \begin{scope}[
                spy using outlines={%
                    zoombox paths,
                    width=\imagewidth / \pgfkeysvalueof{/tikz/zoomboxarray columns} - (\pgfkeysvalueof{/tikz/zoomboxarray columns} - 1) / \pgfkeysvalueof{/tikz/zoomboxarray columns} * \pgfkeysvalueof{/tikz/zoomboxarray inner gap} -\pgflinewidth,
                    height=\imageheight / \pgfkeysvalueof{/tikz/zoomboxarray rows} - (\pgfkeysvalueof{/tikz/zoomboxarray rows} - 1) / \pgfkeysvalueof{/tikz/zoomboxarray rows} * \pgfkeysvalueof{/tikz/zoomboxarray inner gap}-\pgflinewidth,
                    magnification=3,
                    every spy on node/.style={
                        zoombox paths
                    },
                    every spy in node/.style={
                        zoombox paths
                    }
                }
            ]
        },
        execute at end picture={
            \end{scope}
            \node at (image.north) [anchor=north,inner sep=0pt] {\subcaptionbox{\label{\pgfkeysvalueof{/tikz/figurename}-image}}{\phantomimage}};
            \node at (zoomboxes container.north) [anchor=north,inner sep=0pt] {\subcaptionbox{\label{\pgfkeysvalueof{/tikz/figurename}-zoom}}{\phantomimage}};
     \gdef\patternnumber{0}
        },
        spymargin/.initial=1ex,
        zoomboxes xshift/.initial=1,
        zoomboxes right/.code=\pgfkeys{/tikz/zoomboxes xshift=1},
        zoomboxes left/.code=\pgfkeys{/tikz/zoomboxes xshift=-1},
        zoomboxes yshift/.initial=0,
        zoomboxes above/.code={
            \pgfkeys{/tikz/zoomboxes yshift=1},
            \pgfkeys{/tikz/zoomboxes xshift=0}
        },
        zoomboxes below/.code={
            \pgfkeys{/tikz/zoomboxes yshift=-1},
            \pgfkeys{/tikz/zoomboxes xshift=0}
        },
        caption margin/.initial=1ex,
    },
    adjust caption spacing/.code={},
    image container/.style={
        inner sep=0pt,
        at=(image.north),
        anchor=north,
        adjust caption spacing
    },
    zoomboxes container/.style={
        inner sep=0pt,
        at=(image.north),
        anchor=north,
        name=zoomboxes container,
        xshift=\pgfkeysvalueof{/tikz/zoomboxes xshift}*(\imagewidth+\pgfkeysvalueof{/tikz/spymargin}),
        yshift=\pgfkeysvalueof{/tikz/zoomboxes yshift}*(\imageheight+\pgfkeysvalueof{/tikz/spymargin}+\pgfkeysvalueof{/tikz/caption margin}),
        adjust caption spacing
    },
    calculate dimensions/.code={
        \pgfpointdiff{\pgfpointanchor{image}{south west} }{\pgfpointanchor{image}{north east} }
        \pgfgetlastxy{\imagewidth}{\imageheight}
        \global\let\imagewidth=\imagewidth
        \global\let\imageheight=\imageheight
        \gdef\columncount{1}
        \gdef\rowcount{1}
        \gdef\zoomboxcount{1}
    },
    image node/.style={
        inner sep=0pt,
        name=image,
        anchor=south west,
        append after command={
            [calculate dimensions]
            node [image container,subfigurename=\pgfkeysvalueof{/tikz/figurename}-image] {\phantomimage}
            node [zoomboxes container,subfigurename=\pgfkeysvalueof{/tikz/figurename}-zoom] {\phantomimage}
        }
    },
    color code/.style={
        zoombox paths/.append style={draw=#1}
    },
    connect zoomboxes/.style={
    spy connection path={\draw[draw=none,zoombox paths] (tikzspyonnode) -- (tikzspyinnode);}
    },
    help grid code/.code={
        \begin{scope}[
                x={(image.south east)},
                y={(image.north west)},
                font=\footnotesize,
                help lines,
                overlay
            ]
            \foreach \x in {0,1,...,9} { 
                \draw(\x/10,0) -- (\x/10,1);
                \node [anchor=north] at (\x/10,0) {0.\x};
            }
            \foreach \y in {0,1,...,9} {
                \draw(0,\y/10) -- (1,\y/10);                        \node [anchor=east] at (0,\y/10) {0.\y};
            }
        \end{scope}    
    },
    help grid/.style={
        append after command={
            [help grid code]
        }
    },
}

\newcommand\phantomimage{%
    \phantom{%
        \rule{\imagewidth}{\imageheight}%
    }%
}
\newcommand\zoombox[2][]{
    \begin{scope}[zoombox paths]
        \pgfmathsetmacro\xpos{
            (\columncount-1)*(\imagewidth / \pgfkeysvalueof{/tikz/zoomboxarray columns} + \pgfkeysvalueof{/tikz/zoomboxarray inner gap} / \pgfkeysvalueof{/tikz/zoomboxarray columns} ) + \pgflinewidth
        }
        \pgfmathsetmacro\ypos{
            (\rowcount-1)*( \imageheight / \pgfkeysvalueof{/tikz/zoomboxarray rows} + \pgfkeysvalueof{/tikz/zoomboxarray inner gap} / \pgfkeysvalueof{/tikz/zoomboxarray rows} ) + 0.5*\pgflinewidth
        }
        \edef\dospy{\noexpand\spy [
            #1,
            zoombox paths/.append style={
                black and white pattern=\patternnumber
            },
            every spy on node/.append style={#1},
            x=\imagewidth,
            y=\imageheight
        ] on (#2) in node [anchor=north west] at ($(zoomboxes container.north west)+(\xpos pt,-\ypos pt)$);}
        \dospy
        \pgfmathtruncatemacro\pgfmathresult{ifthenelse(\columncount==\pgfkeysvalueof{/tikz/zoomboxarray columns},\rowcount+1,\rowcount)}
        \global\let\rowcount=\pgfmathresult
        \pgfmathtruncatemacro\pgfmathresult{ifthenelse(\columncount==\pgfkeysvalueof{/tikz/zoomboxarray columns},1,\columncount+1)}
        \global\let\columncount=\pgfmathresult
        \ifblackandwhitecycle
            \pgfmathtruncatemacro{\newpatternnumber}{\patternnumber+1}
            \global\edef\patternnumber{\newpatternnumber}
        \fi
    \end{scope}
}

==> math_commands.tex <==


%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Added minimize
\DeclareMathOperator*{\minimize}{minimize}
% Add given
\newcommand\given[1][]{\:#1\vert\:}

% Inline row / column vector
\newcommand{\icol}[1]{% inline column vector
  \left(\begin{smallmatrix}#1\end{smallmatrix}\right)%
}

\newcommand{\irow}[1]{% inline row vector
  \begin{smallmatrix}(#1)\end{smallmatrix}%
}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\bepsilon{{\mathbf{\epsilon}}}
\def\btheta{{\mathbf{\theta}}}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\be{{\mathbf{e}}}
\def\bf{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bu{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\calA{{\mathcal{A}}}
\def\calB{{\mathcal{B}}}
\def\calC{{\mathcal{C}}}
\def\calD{{\mathcal{D}}}
\def\calE{{\mathcal{E}}}
\def\calF{{\mathcal{F}}}
\def\calG{{\mathcal{G}}}
\def\calH{{\mathcal{H}}}
\def\calI{{\mathcal{I}}}
\def\calJ{{\mathcal{J}}}
\def\calK{{\mathcal{K}}}
\def\calL{{\mathcal{L}}}
\def\calM{{\mathcal{M}}}
\def\calN{{\mathcal{N}}}
\def\calO{{\mathcal{O}}}
\def\calP{{\mathcal{P}}}
\def\calQ{{\mathcal{Q}}}
\def\calR{{\mathcal{R}}}
\def\calS{{\mathcal{S}}}
\def\calT{{\mathcal{T}}}
\def\calU{{\mathcal{U}}}
\def\calV{{\mathcal{V}}}
\def\calW{{\mathcal{W}}}
\def\calX{{\mathcal{X}}}
\def\calY{{\mathcal{Y}}}
\def\calZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Theorem environments
% Theorems, definitions, etc
%\def\thmcolon{\hspace{-.85em} {\bf :}}
\def\thmcolon{\relax}

% \newtheorem{THEOREM}{Theorem}
%\newtheorem{THEOREM}{Theorem}[section]
% \newtheorem{LEMMA}[THEOREM]{Lemma}
% \newtheorem{PROPOSITION}[THEOREM]{Proposition}
% \newtheorem{COROLLARY}[THEOREM]{Corollary}
% \newtheorem{DEFINITION}[THEOREM]{Definition}
% \newtheorem{OBSERVATION}[THEOREM]{Observation}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}

% Easiest way to remove the full stop and add a colon
% \usepackage{xpatch}
% \makeatletter
% \AtBeginDocument{\xpatchcmd{\@thm}{\thm@headpunct{.}}{\thm@headpunct{:}}{}{}}
% \makeatother

% \newenvironment{theorem}{\begin{THEOREM} \thmcolon \rm}{\end{THEOREM}}
% \newenvironment{lemma}{\begin{LEMMA} \thmcolon \rm}{\end{LEMMA}}
% \newenvironment{proposition}{\begin{PROPOSITION} \thmcolon \rm}{\end{PROPOSITION}}
% \newenvironment{corollary}{\begin{COROLLARY} \thmcolon \rm}{\end{COROLLARY}}
% \newenvironment{definition}{\begin{DEFINITION} \thmcolon \rm}{\end{DEFINITION}}
% \newenvironment{observation}{\begin{OBSERVATION} \thmcolon \rm}{\end{OBSERVATION}}


%%%%% ABBREVIATIONS %%%%%
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother
